More Than React: Investigating The Role of EmojiReaction in GitHub Pull Requests

Context: Open source software development has become more social and collaborative, especially with the rise of social coding platforms like GitHub. Since 2016, GitHub started to support more informal methods such as emoji reactions, with the goal to reduce commenting noise when reviewing any code changes to a repository. Interestingly, preliminary results indicate that emojis do not always reduce commenting noise (i.e., eight out of 20 emoji reactions), providing evidence that developers use emojis with ulterior intentions. From a reviewing context, the extent to which emoji reactions facilitate for a more efficient review process is unknown. Objective: In this registered report, we introduce the study protocols to investigate ulterior intentions and usages of emoji reactions, apart from reducing commenting noise during the discussions in GitHub pull requests (PRs). As part of the report, we first perform a preliminary analysis to whether emoji reactions can reduce commenting noise in PRs and then introduce the execution plan for the study. Method: We will use a mixed-methods approach in this study, i.e., quantitative and qualitative, with three hypotheses to test.

==> draft.tex <==
% Introduction 
In the past few years, open source software development has become more social and collaborative. Social coding promotes formal and informal collaboration in software development by empowering the exchange of knowledge between developers~\cite{dabbish2012social}.
As one of the most popular platforms, GitHub is the largest collection of open source software in the world, with more than 65 million developers collaborating across 209 million repositories.\footnote{\url{https://github.com/search}}

Every day, thousands of people engage in conversations about code, design, bugs, and new ideas on GitHub. Sometimes, developers want to give simple feedback, and there is no need for a separate comment. Besides, developers have become accustomed to using emojis to represent their emotions. The notable trend is that emojis are not only widely used in regular online communication but are also increasingly used in software development practices, from code in programs to online forums such as Stack Overflow and GitHub~\cite{siadati2017modelling}. Therefore, GitHub has introduced a new social function called ``reaction''. This function is based on ``graphic characters'', which is also the social function of emoji. This function can support developers make simple response on issue, pull request or comment in the GitHub repository. However, little is known about the usage and impact of GitHub reactions from repositories and comments on software development practices.


In this study, we compare the usage of reactions from repositories that are created before and after this feature was introduced.

% To this purpose, we collect and analyze reactions to more than 100 GitHub issues and pull requests, around 359 repositories.

% We show that....


% Background 

In this section, we present the background for existing work related to GitHub reactions.

% Viera and Garrett~\cite{de2020analysis}  
% by using sentiment analysis classifiers to compare GitHub data with other social networks (Twitter and Reddit). By determining that users can provide responses to other user posts on GitHub, and use them as indicators or tags for emotional information, finally showed that there is significant sentiment information contained in non-textually information in the GitHub network. 

Lu et al.\cite{lu2018first} found that emojis are used by quite a few GitHub users. Compared with Internet users, developers have shown interesting usage characteristics and have their own interpretation of the meaning of emoji. In addition, the use of emoji reflects the positive and supportive culture of the community.

GitHub is mainly used as a collaboration platform for software development. On the platform, developers communicate through issues, pull requests, but if the user just wants to make simple feedback, the text will only become too redundant and inefficient. GitHub designers argued that reacting to a comment avoids long threads with many comments lacking relevant content. Hence, In 2016 GitHub introduced a new social feature named Reactions to express their feelings on issues and pull requests quickly.

GitHub provides eight different reactions for use in issues and pull requests in the Figure~\ref{fig:reactions}. Borges et al.\cite{borges2019beyond} present the definition of these six reactions:
Thumbs up, which is used to express acceptance or approval. Thumbs down, which is used to express rejection or disapproval.
Laugh, which indicates a fun situation or happiness. It is also used to express sarcasm or irony in negative situations.
Hooray, which is also used to celebrate or express a happy situation. For example, it is commonly used in software releases.
Confused, which is proposed to express doubt or some difficulty to understand a specific subject.
Heart, which indicates a strong acceptance or approval; it is used when the user really likes something.

Developers can only add one reaction per post (issues or pull requests). Likewise, the reaction can be added to resolved issues and requests. However, project owners can lock issues or pull requests to disable comments and reactions.
